Open-vocabulary Attribute Detection

Vision-language modeling has enabled open-vocabulary tasks where predictions can be queried using any text prompt in a zero-shot manner. Existing open-vocabulary tasks focus on object classes, whereas research on object attributes is limited due to the lack of a reliable attribute-focused evaluation benchmark. This paper introduces the Open-Vocabulary Attribute Detection (OVAD) task and the corresponding OVAD benchmark. The objective of the novel task and benchmark is to probe object-level attribute information learned by vision-language models. To this end, we created a clean and densely annotated test set covering 117 attribute classes on the 80 object classes of MS COCO. It includes positive and negative annotations, which enables open-vocabulary evaluation. Overall, the benchmark consists of 1.4 million annotations. For reference, we provide a first baseline method for open-vocabulary attribute detection. Moreover, we demonstrate the benchmark's value by studying the attribute detection performance of several foundation models. Project page https://ovad-benchmark.github.io

==> figures/att_types_ablation.tex <==
\begin{figure*}[h]
\includegraphics[ width=13cm]{./images/supplementary/att_types_ablation.pdf}
\centering
\caption{Comparison of our baseline method on the type of attributes using different parts-of-caption as proxy-labels.}
\label{fig:att_type_ablation}
\end{figure*}

==> sup_sections/4_model_ablation.tex <==
\subsection{Ablation on the parts-of-caption proxy-labels}
\input{figures/att_types_ablation}
Figure \ref{fig:att_type_ablation} shows the performance per attribute type of the baseline method using different parts-of-caption as proxy-labels, the same models as discussed in Section 5.3. By adding parts-of-caption, \textit{i.e.}, text that includes only nouns/noun phrases/noun complements, the performance improves significantly for 15 out of the 19 attribute types. 
For attributes such as gender, the baseline model shows a high improvement over the chance score when using nouns as proxy-labels, since man/woman and girl/boy include the gender attribute within the noun word. Other attributes like size have a high improvement over the chance prediction when using noun complements as proxy-labels, because in many cases, these noun complements correspond to the attribute words such as small or big. 
The baseline model does not improve over the chance level of the group attribute type. We believe this is because the data distribution is skewed towards bounding boxes with single objects, and 
the words \textit{group} or \textit{single} are less common than the plural version of objects in the captions. 

==> tables/sota_ova_box.tex <==

\begin{table*}[t]\scriptsize
\centering 
\begin{tabular}{ |c|@{\hspace{0.1mm}}c@{\hspace{0.1mm}}|c|ccc|} 
    \hline 
    %Method & All & Head & Medium & Tail \\
    \multirow{2}{*}{Method} & Training & \multicolumn{4}{|c|}{ OVA-BOX } \\
    & Data & All & Head & Medium & Tail \\ 
    \hline
    Chance & - & 8.6 & 36.0 & 7.3 & 0.6 \\
    \hline
    Clip RN50~\cite{clip}  & 400M (10) & 15.8 & 42.5 & 17.5 & 4.2 \\
    Clip VIT-B16~\cite{clip}  & 400M (10) & 16.6 & 43.9 & 18.6 & 4.4 \\
    \hline
    Open Clip RN50~\cite{open_clip}  & 12M (8b) & 11.8 & 41.0 & 11.7 & 1.4 \\
    %Open Clip RN50~\cite{open_clip}  & 15M (9) & 11.8 & 41.1 & 11.8 & 1.4 \\
    Open Clip ViT-B16~\cite{open_clip}  & 400M (9b) & 16.0 & 45.4 & 17.4 & 3.8 \\
    Open Clip ViT-B32~\cite{open_clip}  & 2B (9c) & 17.0 & 44.3 & 18.4 & 5.5 \\
    \hline
    ALBEF~\cite{albef}  & 4M (1a,4,5,8a) & 15.6 & 43.1 & 17.3 & 3.7 \\
    ALBEF~\cite{albef}  & 14M (1a,4,5,8) & 15.3 & 43.7 & 17.1 & 3.0 \\
    ALBEF~\cite{albef}  & 14M (1a,4,5,8) + ft(1a) & 18.3 & 44.9 & 21.1 & 5.3 \\
    ALBEF~\cite{albef}  & 14M (1a,4,5,8) + ft(3) & 20.4 & 46.9 & 23.5 & 7.2 \\
    ALBEF~\cite{albef}  & 14M (1a,4,5,8) + ft(2) & 21.0 & 44.2 & 23.9 & 9.4 \\
    \hline
    Blip~\cite{blip}  & 14M (1a,4,5,8) & 17.0 & 46.6 & 18.3 & 5.0 \\
    Blip~\cite{blip}  & 129M (1a,4,5,8,9a) & 18.2 & 44.4 & 20.7 & 5.7 \\
    Blip~\cite{blip}  & 129M (1a,4,5,8,9a) + ft(2) & 23.3 & 50.2 & 26.8 & 9.5 \\
    Blip~\cite{blip}  & 129M (1a,4,5,8,9a) + ft(1a) & 24.3 & 51.0 & 28.5 & 9.7 \\
    \hline
    X-VLM~\cite{xvlm}  & 16M (1$^{*}$,4$^{*}$,5,6$^{*}$,7$^{*}$,8) + ft(1a) & 25.0 & \textbf{54.2} & 30.6 & 7.7 \\
    X-VLM~\cite{xvlm}  & 4M (1$^{*}$,4$^{*}$,5,8a) + ft(1a) & 25.5 & 52.6 & 31.2 & 8.8 \\
    X-VLM~\cite{xvlm}  & 4M (1$^{*}$,4$^{*}$,5,8a) & 25.9 & 50.3 & 32.0 & 9.8 \\
    X-VLM~\cite{xvlm}  & 16M (1$^{*}$,4$^{*}$,5,6$^{*}$,7$^{*}$,8) + ft(2) & 26.2 & 48.7 & 31.2 & 12.1 \\
    X-VLM~\cite{xvlm}  & 4M (1$^{*}$,4$^{*}$,5,8a) + ft(2) & 27.6 & 49.8 & 33.2 & 12.8 \\
    X-VLM~\cite{xvlm}  & 16M (1$^{*}$,4$^{*}$,5,6$^{*}$,7$^{*}$,8) & \textbf{28.1} & 49.7 & \textbf{34.2} & \textbf{12.9} \\
    \hline
    \modelname- Box  & 0.11M (1a,1b$^{*\text{base}}$) & 21.4$\pm$0.4 & 48.0$\pm$0.5 & 26.9$\pm$0.6 & 5.2$\pm$0.5 \\
    \hline
\end{tabular}
\caption{Open-Vocabulary Attribute Detection results (mAP) in the box-oracle setting. $^{*}$: models use the localization information in the annotations of this dataset.}
\label{tab:ova_sota_box}
\end{table*}

% Datasets
% COCO captions - T:118287 - V:5000
% COCO object detection - T:118287 - V:5000
% COCO captions - 550K
% COCO and VG are datasets extracted from Flickr

% VG
% objects 2516939
% regions 5408689
% relationships 2316104
% attributes 3802374

\begin{table}[]\scriptsize
    \centering
    \begin{tabular}{|rl|cccc|}
        \hline 
        \# & Dataset         & \#Images  & \#Captions    & \#Objects     & \#Regions \\
        \hline 
        (1a) & COCO Captions   & 0.12M   & 0.57M       & -             & -         \\
        (1b) & COCO Objects    & 0.12M   & -           & 0.86M         & -         \\
        (2) & RefCOCO+        & 0.019M  & -           & -             & 0.14M   \\
        % (2) & RefCOCO+        & 0.019M  & -           & -             & 141,564   \\
        (3) & Flickr30K       & 0.029M  & -           & 0.86M         & -         \\
        (4) & VG              & 0.10M   & -           & 2.5M          & 5.4M      \\
        (5) & SBU Captions    & 1M      & 1M          & -             & -         \\
        (6) & OpenImages      & 1.7M    & 0.67M       & 4.4M          & 3.3M      \\
        (7) & Objects365      & 1.8M    & -           & 29M           & -         \\
        (8a) & CC-3M          & 2.95M   & 2.95M       & -             & -         \\
        (8b) & CC-12M         & 11.1M   & 11.1M       & -             & -         \\
        %(9) & YFCC100M       & 99.2M   & 99.2M       & -             & -         \\
        (9a) & LAION         & 115M    & 115M        & -             & -         \\
        (9b) & LAION         & 400M    & 400M        & -             & -         \\
        (9c) & LAION         & 2B      & 2B          & -             & -         \\
        (10) & CLIP 400M      & 400M    & 400M        & -             & -         \\
        \hline 
    \end{tabular}
    \caption{Training set legend and statistics.}
    \label{tab:my_label}
\end{table}{}

